Gluing variations

We establish several results on gluing/embedding/extending geometric structures in vacuum spacetimes with a cosmological constant in any spacetime dimensions $d\ge 4$, with emphasis on characteristic data. A useful tool is provided by the notion of submanifold-data of order $k$. As an application of our methods we prove that vacuum Cauchy data on a spacelike Cauchy surface with boundary can always be extended to vacuum data defined beyond the boundary.

==> JHmacros.tex <==
\newcommand{\mcB}{{\mathcal B}}


\def\ft#1#2{{\textstyle{{\scriptstyle #1}\over {\scriptstyle #2}}}}
\def\fft#1#2{{#1 \over #2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Q#1#2{\frac{\partial #1}{\partial #2}}
\def\d{\partial}
\def\QS#1#2{\frac{\partial^S #1}{\partial #2}}
\def\varQ#1#2{\frac{\delta #1}{\delta #2}}
\def\varQL#1#2{\frac{\delta^L #1}{\delta #2}}
\def\norm#1{\|#1\|}
\def\eps{\epsilon}
\def\vareps{\varepsilon}
\def\radg{\sqrt{-g}}
\def\dnx{\hspace{0.06em}\text{d}^n \hspace{-0.06em} x}
\def\dv{\text{d}_V}
\def\dx{\text{d}\hspace{-0.06em}x}
\def\dvphi{\text{d}_V\hspace{-0.06em}\phi}
\def\dvxi{\text{d}_V\hspace{-0.06em}\xi}
\def\half{\frac{1}{2}}

\def\no{\nonumber}
\def\beq{\begin{eqnarray}}
\def\eeq{\end{eqnarray}}
\def\mathun{\hbox{ 1\hskip -3pt l}}
\def \RR{{\mathbb{R}}}
\def \C{{\mathbb{C}}}
\def \NN{{\mathbb{N}}}
\def\sst#1{{\scriptscriptstyle #1}}
\def\ie{{\it i.e.~}}
\def\mf{\mathfrak}
%%%% lettres greques %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\a{\alpha}
\def\b{\beta}
\def\c{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\f{\sigma}
\def\h{\eta}
\def\k{\kappa}
\def\La{\red{\Lambda}}
\def\G{\Gamma}
\def\D{\Delta}
\def\m{\mu}
\def\n{\nu}
\def\r{\rho}
\def\o{\omega}
\def\O{\Omega}
\def\S{\Sigma}
\def\t{\tau}
\def\th{\theta}
\def\p{\pi}
\def\ve{\varepsilon}
\def\x{\xi}
\def\z{\zeta}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}



==> LambdaMacros.tex <==
\newcommand{\refq}{\mnote{blue text added or changed following a query from a referee}\color{blue}}



{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{figure}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{table}{section}
\renewcommand{\thetable}{\thesection.\arabic{table}}


\newcommand{\ovg}{\red{\overline{{g}}}}
\newcommand{\og}{\ovg}

\newcommand{\mybar}[1]{\blue{\check{#1}}}

\newcommand{\tautheta}{\thetatau}

\newcommand{\genK}{L}%
\newcommand{\prd}{\frac 1 {\msqh} \partial_r \Big(\msqh\Big)}%
\newcommand{\genL}{\underbar{{\mbox{\emph L}}}\,}%


\newcommand{\eendxone}{\blue{\rho}}
\newcommand{\eendxtwo}{\blue{\underline{\rho}}}


\newcommand{\ob}[1]{\overline{#1}}
\newcommand{\ts}[1]{\text{TS}{\big[#1\big]}}
\newcommand{\pt}[1]{\phantom{#1}}


\newcommand{\eendx}{\blue{\rho}}

\newcommand{\thetatau}{\blue{\theta}}
\newcommand{\uthetatau}{\blue{\underline{\theta}}}

\newcommand{\tthetatau}{\blue{\tilde\theta}}
\newcommand{\tuthetatau}{\blue{\underline{\tilde{\theta}}}}

\newcommand{\umcN}{\blue{\underline{\mcN}}}

\newcommand{\Ione}{\blue{I}}
\newcommand{\Itwo}{\blue{\underline{I}}}

\newcommand{\subman}{\blue{{\mathcal J}}}
\newcommand{\mcNone}{\blue{\mcN}}
\newcommand{\mcNtwo}{\umcN}


\newcommand{\mcNonep}{\mcNone_{[0,1]}}
\newcommand{\mcNtwop}{\umcN_{[0,1]}}

\newcommand{\mcNonem}{\mcNone_{[-1,0]}}
\newcommand{\mcNtwom}{\umcN_{[-1,0]}}


\newcommand{\usecN}{\blue{\underline{\secN}}}

\newcommand{\xone}{\blue{u}}
\newcommand{\xtwo}{\blue{\underline{u}}}

\newcommand{\btdv}{\blue{\tilde{\underline{u}}}}
\newcommand{\mtdx}{\blue{\check x}}%{\tilde x}
\newcommand{\mtdg}{\blue{\check g}}%{\tilde x}
\newcommand{\mtdv}{\blue{\check v}}
\newcommand{\mtdu}{\blue{\check u}}%{\tilde u}
\newcommand{\mtdr}{\blue{\check r}}%{\tilde r}
\newcommand{\mtdA}{\blue{\check A}}%{\tilde A}
\newcommand{\mtdB}{\blue{\check B}}%{\tilde B}
\newcommand{\mtdC}{\blue{\check C}}%{\tilde C}

\newcommand{\kN}{\blue{k\in\N\cup\{\infty\}}}

\newcommand{\ClS}{\blue{C^\ell_{\secN^\perp} C^\infty_{\secN^\parallel}}}
\newcommand{\CkS}{\blue{C^k_{\secN^\perp} C^\infty_{\secN^\parallel}}}

\newcommand{\CSdataBo}[1]{{\blue{\Psi_{\mathrm{Bo}}[#1]}}{}}
\newcommand{\CSdataIM}[1]{{\blue{\Psi_{\mathrm{IM}}[#1]}}{}}
\newcommand{\CSdata}[1]{{\blue{\Psi[#1]}}{}}
\newcommand{\tCSdata}[1]{{\blue{\tilde{\Psi}[#1]}}{}}

\newcommand{\CdataBo}[1]{{\blue{\Phi_{\mathrm{Bo}}[#1]}}{}}
\newcommand{\CdataIM}[1]{{\blue{\Phi_{\mathrm{IM}}[#1]}}{}}
\newcommand{\Cdata}[1]{{\blue{\Phi[#1]}}{}}
\newcommand{\tCdata}[1]{{\blue{\tilde{\Phi}[#1]}}{}}

\newcommand{\TSzlap}{\blue{\Delta_{\ringh}}}%{\blue{\mathring \triangle}}
\newcommand{\zDelta}{\TSzlap}

\newcommand{\noCdata}[1]{\CSdata{#1}}

\newcommand{\ua}{{\underline{\alpha}}{}}
\newcommand{\ualpha}{{\ua}}
\newcommand{\ualp}{{\ua}}
\newcommand{\bb}{{\underline{\beta}}{}}
\newcommand{\ub}{{\bb}}
\newcommand{\ubeta}{{\bb}}
%\renewcommand{\a}{\alpha}
%\renewcommand{\b}{\beta}
\newcommand{\dual}{\mbox{}^{\star}\!}
\newcommand{\rdual}{^{\star}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\si}{\sigma}
\newcommand{\sii}{\bar{\sigma}}
\newcommand{\ro}{\rho}
\newcommand{\roo}{\bar{\ro}}
\newcommand{\ze}{\zeta}
\newcommand{\hze}{\hat\zeta}

\newcommand{\alp}{\alpha}

\newcommand{\obe}{\mathring{\beta}}
\newcommand{\obeta}{\obe}
\newcommand{\obetab}{\oubeta}
\newcommand{\oube}{\,\,\mathring{\!\!\ubeta}}
\newcommand{\oubeta}{\oube}
\newcommand{\osi}{\mathring{\sigma}}
\newcommand{\osigma}{\osi}
\newcommand{\orho}{\mathring{\rho}}
\newcommand{\oro}{\orho}
\newcommand{\ups}{\upsilon}
\newcommand{\upsb}{\underline{\upsilon}}
\newcommand{\hups}{\hat{\ups}}
\newcommand{\hupsb}{\hat{\upsb}}


\newcommand{\fourg}{\red{\mathbf{g}}}

\newcommand{\zdiv}{\blue{\operatorname{\mathring{\text div}}\,}}
\newcommand{\zdivtwo}{\blue{\operatorname{\mathring{\text div}_{(2)}}\,}}
\newcommand{\zdivone}{\blue{\operatorname{\mathring{\text div}_{(1)}}\,}}

\newcommand{\Lop}{\operatorname{\red{L}}}
\newcommand{\hLop}{\widehat{\operatorname{\red{ L}}}}

\newcommand{\whmcN}[1]{\blue{{\umcN}_{\, #1}}}
\newcommand{\hmcN}[1]{\,\,\,\,\,\blue{\widehat{\!\!\!\!\!{\mcN}_{\, #1}}}}

\newcommand{\thyp}[1]{\blue{\,\widetilde{\!\,\hyp}_{\, #1}}}
\newcommand{\tmcN}[1]{\blue{\,\,\,\,\widetilde{\!\!\!\!\mcN_{\, #1}}}}
\newcommand{\wmcL}{{\,\,\,\widetilde{\!\!\!\mcL}}}
\newcommand{\wmcH}{{\,\,\,\widetilde{\!\!\!\mcH}}}


\newcommand{\Vect}{\blue{\mathop{\mathrm{Vect}}}}

\newcommand{\TS}{\mathop{\mathrm{TS}}}
\newcommand{\rbox}[1]{\fbox{\blue{$#1$}}}
\newcommand{\bbox}[1]{\fbox{\blue{$#1$}}}

\newcommand{\guu}{\blue{g_{uu}}}
\newcommand{\twoscsign}{{\blue{\varepsilon}}}

\newcommand{\interph}{\blue{v}}

\newcommand{\overadd}[2]{\overset{\mbox{\tiny (#1)}}{#2}}

\newcommand{\cDelta}{\blue{\Delta}}

\newcommand{\psiP}{\blue{\psi}}



\newcommand{\tkfbd}{\blue{\mathrm{b.d.}|_{r_1}}}
\newcommand{\tk}{\tkfbd}

\newcommand{\secN}{\blue{\mathbf{S}}}

\newcommand{\HS}[1]{\blue{H_{k_{#1}}(\secN)}}
\newcommand{\HSm}[1]{\blue{H_{k_{#1}-1}(\secN)}}
\newcommand{\HSmtwo}[1]{\blue{H_{k_{#1}-2}(\secN)}}

\newcommand{\Hgamma}{\blue{H_{k_\gamma}(\secN)}}
\newcommand{\Hgammar}{\blue{H_{k_{\partial_r\gamma}}(\secN)}}
\newcommand{\HV}{\blue{H_{k_V}(\secN)}}
\newcommand{\Hbeta}{\blue{H_{k_\beta}(\secN)}}
\newcommand{\HU}{\blue{H_{k_U}(\secN)}}
\newcommand{\HUr}{\blue{H_{k_{\partial_r U}}(\secN)}}



\newcommand{\momega}{\blue{\mu }}
\newcommand{\Bpsi}{\blue{\psi}}

\newcommand{\referee}{}%{\mnote{change as suggested by the referee}
%\color{blue}{}}
\newcommand{\refer}{\mnote{change as suggested by the referee}
\color{blue}{}}

\newcommand{\wh}{\blue{w}}

\newcommand{\red}[1]{{\color{red} #1}}

\newcommand{\ringzeta}{{  \mathring \zeta}}

\newcommand{\bluec}{\color{blue}}
\newcommand{\barh}{\blue{ h }}%{\blue{ h^{\mathrm{reg}}}}
\newcommand{\hBo}{\blue{ h^{\mathrm{Bo}}}}

\newcommand{\Vol}{{V}}%\mathrm{Vol}}

\newcommand{\nopmass}{{\color{red}m^2}}
%\newcommand{\pmass}{{\color{blue}+m^2}}
\newcommand{\pmass}{{+m^2}}
\newcommand{\mmass}{{\color{blue}-m^2}}

\newcommand{\inu}{{\color{blue} \nu}}


\newcommand{\omthree}[1]{\overset{\mbox{\tiny (-3)}}{#1}}

\newcommand{\omtwo}[1]{\overset{\mbox{\tiny (2)}}{#1}}
\newcommand{\omone}[1]{\overset{\mbox{\tiny (1)}}{#1}}
\newcommand{\ozero}[1]{\overset{\mbox{\tiny (0)}}{#1}}
\newcommand{\otwoone}[1]{\overset{\mbox{\tiny (-2,1)}}{#1}}
\newcommand{\othreeone}[1]{\overset{\mbox{\tiny (-3,1)}}{#1}}
\newcommand{\otwo}[1]{\overset{\mbox{\tiny (-2)}}{#1}}
\newcommand{\othree}[1]{\overset{\mbox{\tiny (-3)}}{#1}}
\newcommand{\ofour}[1]{\overset{\mbox{\tiny (-4)}}{#1}}
\newcommand{\oone}[1]{\overset{\mbox{\tiny (-1)}}{#1}}
\newcommand{\ok}[1]{\overset{\mbox{\tiny (-k)}}{#1}}


\newcommand{\edS}{\, \blue{=\!\big|_{g=\mathring g}}\, }

\newcommand{\hdpot}{\blue{\hat \chi}}
\newcommand{\hrotpot}{\blue{\check \chi}}

\newcommand{\zTSxi}{\blue{\mathring \xi}}

\newcommand{\TB}{\blue{\mathrm{TB}}}

\newcommand{\breh}{\blue{\breve{h}}}

\newcommand{\IntPsi}{{\mathring \Ipsi}}

\newcommand{\deltag}{\blue{\blue{h}}}
\newcommand{\btheta}{\blue{\mathbf{\theta}}}
\newcommand{\ctau}{\blue{\tau}}
\newcommand{\tg}{\blue{\tilde{g}}}
\newcommand{\hg}{\blue{\tilde{g}}}
\newcommand{\hnabla}{\blue{\hat{\nabla}}}
\newcommand{\tform}{{\blue{\tilde{\eta}}}}
\newcommand{\ztR}{{\blue{\mathring{\tilde R}}}}

  \newcommand{\mypi}{{\pi}}
  \newcommand{\tpi}{{\tilde\mypi}}
  \newcommand{\tphi}{{\tilde\phi}}
  \newcommand{\bmetric}{{b}}

\newcommand{\R}{\mathbb{R}}

\newcommand{\olive}{\color{olive}}
%\newcommand{\purple}{\color{purple}}
\newcommand{\purple}{}

\newcommand{\limatrzero}{{\lim_{ r\to r_0}}}%
\newcommand{\intfromrzero}{\int_{r=r_0}}%
\newcommand{\psintfromrzero}{\int_{s'= 0}}%
\newcommand{\sintfromrzero}{\int_{s= 0}}%
\newcommand{\pintfromrzero}{\int_{r'=r_0}}%
\newcommand{\tintfromrzero}{\int_{\tilde r=r_0}}%
%


\newcommand{\Ichi}{{\mu}}
\newcommand{\Ipsi}{{\lambda}}


\newcommand{\nodanger}{}
\newcommand{\dangerous}{{\fontencoding{U}\fontfamily{futs}\selectfont\char 66\relax}}
\newcommand{\mdanger}{\danger}%{\mbox{\dangerous}}
\newcommand{\danger}{\mbox{{\dangerous}}}
\newcommand{\CHringh}{{{\breve{h}}}\mbox{\mdanger}}

\newcommand{\lapseTB}{\blue{N}}

\newcommand{\deltaU}{{ {\zhTB}_{u}{}} }

%{{{\delta U}}}

\newcommand{\mcD}{{\mycal D}}

\newcommand{\ud}[2]{^{#1}_{\phantom{#1 } #2}}
\newcommand{\du}[2]{_{#1}^{\phantom{#1 } #2}}
\newcommand{\zhTB}{\blue{\check h}}
\newcommand{\zhTBlog}{\blue{{}^{l}\check h}}
\newcommand{\zhTBW}{\blue{\gamma}}
\newcommand{\zzhTBW}{\blue{\mathring{\zhTBW}}}


\newcommand{\zh}{{\zzhTBW }}
\newcommand{\tetrad}[1]{{\hat{#1}}}
\newcommand{\tetA}{\tetrad{A}}


\newcommand{\TimelikeQ}{{Q}}


 \newcommand{\NullQ}{{Q}}
 \newcommand{\tNullQ}{{\tilde q}}

\newcommand{\tQ}{{\tilde Q}}

\newcommand{\mcO}{{\mycal O}}
\newcommand{\mcU}{{\mycal U}}
\newcommand{\mcM}{{\mycal M}}
\newcommand{\mcN}{{\mycal N}}
 \newcommand{\mcK}{{\mycal K}}
%
\newcommand{\sectionofScri}%
{{ \,\,\,\,\mathring{\!\!\!\!\mcN}}}
%{{\color{red} \,\,\,\,\overline{\!\!\!\!\mcN}\cap\scri}}
\newcommand{\clmcN}{{  \,\,\,\,\overline{\!\!\!\!\mcN}}}
%{{{\color{red} \mathring M TO CHANGE???}}}
\newcommand{\sectionofscri}{\sectionofScri}
\newcommand{\sectionfofscri}{\sectionofScri}


\newcommand{\Mcheckhere}{{ \check N}}
\newcommand{\HMsection}{S^{\tetrad 1}\times \Mcheckhere}
\newcommand{\Mcheck}{\check M}

\newcommand{\Bobig}{{}}%{{\mbox{\rm\scriptsize Bo}}}
\newcommand{\BoBig}{\Bobig}
\newcommand{\Bo}{\Bobo}%{{\mbox{\rm\scriptsize Bo}}}
\newcommand{\Bobo}{{}}%{\mathrm{Bo}}%{{\mbox{\rm\tiny Bo}}}
%\newcommand{\Bobo}{{\mbox{\rm\tiny Bo}}}
%\newcommand{\Bobo}{\textrm{Bo}}%{{\mbox{\rm\tiny Bo}}}


\newcommand{\Bh}{{\mbox{\rm\scriptsize Bh}}}
\newcommand{\Bht}{{\mbox{\rm\tiny Bh}}}

\newcommand{\HM}{{\mbox{\rm\scriptsize HM}}}
\newcommand{\HMt}{{\mbox{\rm\tiny HM}}}



\newcommand{\ourU}{\mathbb U}%

\newcommand{\Kp}{{\mathfrak{g}}}
\newcommand{\Bgamma}{{B}}


\newcommand{\backg}{{b}}
 \newcommand{\dlambda}[1]{{{d #1}\over {d\lambda}}}
 \newcommand{\dtwolambda}[1]{{{d^2 #1}\over {d\lambda^2}}}

 \newcommand{\tomega}{{\tilde \omega}}
 \newcommand{\hyp}{{\mycal S}}
\newcommand{\mcL}{{\mycal L}}
\newcommand{\fullg}{{\mathbf{g}}}%{{}^{n+1}{g}}


\newcommand{\rbo}{r_{\Bo}}
\newcommand{\rBo}{\rbo}

\newcommand{\betaBondi}{\omega}%{{\color{red}\omega}}%

\newcommand{\sigmaaf}{\sigma}
\newcommand{\sigmaafAB}{\sigma_A {}^{ B}}
\newcommand{\sigmabo}{\sigma^{\Bo}{}}
\newcommand{\sigmaboAB}{\sigma^{\Bo}{}\!_A {}^{ B}}

\newcommand{\scri}{{\mycal I}}%
\newcommand{\scrip}{\scri^{+}}%
\newcommand{\scrim}{\scri^{-}}%
\newcommand{\scripm}{\scri^{\pm}}%
\newcommand{\scrp}{{\mycal I}^{+}}%
\newcommand{\Scri}{\scri}


\newcommand{\wascalO}{{O }}
%\newcommand{\wascalO}{{\color{red} O }}
\newcommand{\wascalOof}{{\wasCalOof}}
\newcommand{\wasCalOof}{\redOof}
%\newcommand{\redOof}{{ {O(}}}
\newcommand{\redOofO}{ {O(}}%{{\color{blue} {O(}}}
\newcommand{\redOofo}{{ {o(}}}
\newcommand{\redOof}{{ {O(}}}
\newcommand{\wascalredOof}{\redOof}
%
%:
%
\newcommand{\ellhere}{{  L}}%

 \newcommand{\chitwo}{{  \iota}}
% conformally rescaled real metric
\newcommand{\hhere}{{  \tilde g}}
%{{\color{blue}\lambda}}%
\newcommand{\ringlambda}{{\mathring\hhere}}%
\newcommand{\ringh}{{  \zzhTBW }}%
%


\newcommand{\greenc}{\color{darkgreen}}
\newcommand{\greenca}[1]{\color{darlgreen}\ptcr{change or addition or rewording on #1}}


\newcommand{\redc}{\color{red}}
\newcommand{\blueca}[1]{\color{blue}\ptcr{change or addition or rewording on #1}}
\newcommand{\redca}[1]{\color{red}\ptcr{change or addition or rewording on #1}}
\newcommand{\HLhere}{{  H}}%
%
\newcommand{\renm}{{\mbox{\rm\scriptsize ren}}}

\newcommand{\mTB}{m_{\mbox{\rm\scriptsize TB}} }
\newcommand{\muTB}{{\mu_{\mbox{\rm\scriptsize TB}}}}

\newcommand{\Affr}{{\rho}}

\newcommand{\hring}{\mathring{h}}
\newcommand{\hringmeasure}{d \mu_{\zzhTBW }}
\newcommand{\hringvolume}{\mu_{\zzhTBW }(\sectionofScri)}



\newcommand{\nuoa}{\nuoasymptoticvalue}
\newcommand{\nuAa}{\nuAasymptoticvalue}
\newcommand{\nuBa}{\nuBasymptoticvalue}
\newcommand{\nuoasymptoticvalue}{\left(\nu^{ 0}_\Bo\right)_{ 0}}
\newcommand{\nuAasymptoticvalue}{\left(\nu^A_\Bo\right)_{ 0}}
\newcommand{\nuBasymptoticvalue}{\left(\nu^B_\Bo\right)_{ 0}}


\newcommand{\tr}{\mbox{tr}}
\newcommand{\zg}{\mathring{g}}
\newcommand{\zG}{\mathring{\Gamma}}
\newcommand{\znabla}{ {\mathring{\nabla}}}

\newcommand{\zR}{\blue{\mathring{R}}}



\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\ga}{{\gamma}}
\newcommand{\Mext}{M_\ext}
\newcommand{\ext}{\mathrm{ext}}
\newcommand{\trg}{{\mathrm{tr}_g}}
\newcommand{\divE}{\mathrm{div}(E)}
\newcommand{\divB}{\mathrm{div}(B)}

\newcommand{\Charmass}{Characteristic mass}
\newcommand{\charmass}{characteristic mass}

\newcommand{\noalpha}{{{\varphi}}}
\newcommand{\nobeta}{{{\psi}}}
\newcommand{\nosigma}{{{\chi}}}

\newcommand{\coneg}{\check g}
\newcommand{\coneGamma}{\check \Gamma}
\newcommand{\conenabla}{{\check \nabla}}
\newcommand{\coneR}{\check R}
\newcommand{\aff}{\mathrm{O}}
\newcommand{\ezero}{\overset{\mbox{\tiny 0}}{e}}

\newcommand{\noomega}{{w}}

\newcommand{\meter}{\mathrm{m}}
\newcommand{\myepsilon}{ {\mathring\varepsilon}}

\newcommand{\redad}[2]{\blue{\ptc{change or addition or rewording on #1} #2}}

\newcommand{\nomathringB}{{B}}
\newcommand{\nomathringA}{{A}}
\newcommand{\mathringB}{{\mathring B}}%{{ \danger B}}%
\newcommand{\mathringA}{{\mathring A}}

\newcommand{\smalle}{{ {\mathfrak{e}}}}
\newcommand{\smallh}{{ {\mathfrak{h}}}}

\newcommand{\noatwo}{ {{\beta_1}}}%{{\xout{a_2}}}
\newcommand{\atwo}{ {{(-2)}}}
\newcommand{\plusatwo}{ {{-2}}}
\newcommand{\plustwoatwo}{ {{-4}}}
\newcommand{\minusatwo}{ {{+2}}}
\newcommand{\aonesquared}{{{\psi_{\tetrad 0}^2}}}%{{{\psi_{\tetrad 0}^2}}\danger}
\newcommand{\aone}{ {{\psi_{\tetrad 0}}}}%{{{\psi_{\tetrad 0}}}\danger}

\newcommand{\BobbyE}{{\mycal E}}%
\newcommand{\BobbyB}{{\mycal B}}


\newcommand{\deltaZH}{ {\delta Z_H}}
\newcommand{\deltaZE}{ {\delta Z_E}}

\newcommand{\rout}[1]{{\xout{#1}}}

\newcommand{\eeal}[1]{\label{#1}\end{eqnarray}}

\newtheorem{theorem}{\sc  Theorem\rm}[section]
\newtheorem{acknowledgement}[theorem]{\sc  Acknowledgement\rm}
\newtheorem{algorithm}[theorem]{\sc  Algorithm\rm}
\newtheorem{axiom}[theorem]{\sc  Axiom\rm}
\newtheorem{Theorem}[theorem]{\sc  Theorem\rm}
\newtheorem{thm}[theorem]{\sc  Theorem\rm}
%\newtheorem{case}[theorem]{\sc  Case\rm}
\newtheorem{claim}[theorem]{\sc  Claim\rm}
\newtheorem{conclusion}[theorem]{\sc  Conclusion\rm}
\newtheorem{condition}[theorem]{\sc  Condition\rm}
\newtheorem{conjecture}[theorem]{\sc  Conjecture\rm}
\newtheorem{corollary}[theorem]{\sc  Corollary\rm}
\newtheorem{Corollary}[theorem]{\sc  Corollary\rm}
\newtheorem{criterion}[theorem]{\sc  Criterion\rm}
\newtheorem{definition}[theorem]{\sc  Definition\rm}
\newtheorem{example}[theorem]{\sc  Example\rm}
\newtheorem{exercise}[theorem]{\sc  Exercise\rm}
\newtheorem{lemma}[theorem]{\sc Lemma\rm}
\newtheorem{Lemma}[theorem]{\sc Lemma\rm}

% \theoremstyle{remark}
\newtheorem{notation}[theorem]{\sc Notation\rm}
\newtheorem{problem}[theorem]{\sc Problem\rm}
\newtheorem{proposition}[theorem]{\sc Proposition\rm}
\newtheorem{Proposition}[theorem]{\sc Proposition\rm}
\newtheorem{remark}[theorem]{\sc Remark\rm}
\newtheorem{Remark}[theorem]{\sc Remark\rm}
\newtheorem{Remarks}[theorem]{\sc Remarks\rm}
\newtheorem{remarks}[theorem]{\sc Remarks\rm}
\newtheorem{solution}[theorem]{\sc Solution\rm}
\newtheorem{summary}[theorem]{\sc Summary\rm}
\newtheorem{question}[theorem]{\sc Question\rm}




\DeclareFontFamily{OT1}{rsfs}{}
\DeclareFontShape{OT1}{rsfs}{m}{n}{ <-7> rsfs5 <7-10> rsfs7 <10-> rsfs10}{}
\DeclareMathAlphabet{\mycal}{OT1}{rsfs}{m}{n}


\newcommand{\mnote}[1]
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize $%\!\!\!\!\!\!\,
\bullet$\themnotecount}}$ \marginpar{%\color{red}%
\raggedright\tiny\em $\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }
\newcommand{\mwp}[1]{\mnote{{\bf Bobby:} #1}}

\newcommand{\zgamma}{\blue{\mathring \gamma}}

\newcommand{\mmr}[1]{\mnotex{{\bf mm:} {\color{violet} #1}}}

\newcommand{\mm}[1]{\mnotex{{\bf mm:} {\color{violet} #1}}}

\newcommand{\nonef}{n_1^{\textrm{eff}}}
\newcommand{\ntwof}{n_2^{\textrm{eff}}}


\newcommand{\Z}{\mathbbm{Z}}

\newcommand{\blue}[1]{{\color{blue}#1}}


\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}

\newcommand{\green}[1]{{\color{caribbeangreen} #1}}

\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}



\newcommand{\dire}{ {e}}
\newcommand{\dirb}{ {b}}
\newcommand{\dird}{ {d}}
\newcommand{\dirh}{ {h}}

\newcommand{\blueE}{E}%{\blue{E}}%{\blue{{\textswab{E}}}}%{\blue{{\varmathbb{E}}}} % varmathbb needs txfonts, which produces a terrible font for the whole document
\newcommand{\blueB}{B}%{\blue{B}}%{\blue{{\textswab{B}}}}%{\blue{{\varmathbb{B}}}}

\newcommand{\Ered}{{\mathscr{E}}}
\newcommand{\redE}{\Ered}
\newcommand{\Bred}{{\mathscr{B}}}
\newcommand{\redB}{\Bred}
\newcommand{\Egreen}{\green{\mathds E}}
\newcommand{\greenB}{\green{\mathds B}}
\newcommand{\Dgreen}{\green{\mathds D}}
\newcommand{\greenD}{\Dgreen}
\newcommand{\Bgreen}{\greenB}
\newcommand{\greenH}{\Hgreen}
\newcommand{\Hgreen}{\green{\mathds H}}
\newcommand{\zepsilon}{\blue{\mathring{\epsilon}}}

\newcommand{\griem}{\blue{g}}
\newcommand{\Driem}{\blue{\mathcal D}}

\newcommand{\glorentz}{{\mathbf g}}
\newcommand{\Dlorentz}{{\nabla}}

\newcommand{\ol}[1]{\overline{#1}}


\newcommand{\reda}[1]{\ptcr{addition or rewording or rearrangement}{ #1}}
\newcommand{\added}[2]{\ptcr{addition or rewording or rearrangement on #1 }{ #2}}

\newcommand{\reject}{\ptcr{remove eject}\clearpage}
\newcommand{\mysigma}{{{\sigma}}}

\newcounter{mnotecount}[section]

\renewcommand{\themnotecount}{\thesection.\arabic{mnotecount}}

\newcommand{\mnotex}[1]%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
$%\!\!\!\!\!\!\,
\bullet$\themnotecount}}$ \marginpar{%\color{red}%
\raggedright\tiny\em
$\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }

\newcommand{\ptc}[1]{\mnotex{{\bf ptc:} {  #1}}}
\newcommand{\ptcrr}[1]{\mnotex{{\bf ptc:} {  #1}}}
\newcommand{\ptcr}[1]{\mnotex{{\bf ptc:} {\color{red} #1}}}
\newcommand{\ptcn}[1]{\mnotex{  {\color{blue} #1}}}
\newcommand{\Christopher}[1]{\mnotex{{\bf Christopher:} {\color{red} #1}}}

\newcommand{\change}[1]{{\color{red} #1}\ptcr{changed}}
\newcommand{\add}[1]{{\color{red} #1}\ptcr{added}}

\newcommand{\bel}[1]{\begin{equation}\label{#1}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\bean}{\begin{eqnarray}\nonumber}
\newcommand{\beal}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\nn}{\nonumber}
\newcommand{\Eq}[1]{Equation~\eq{#1}}
\newcommand{\Eqsone}[1]{Equations~\eq{#1}}
\newcommand{\Eqs}[2]{Equations~\eq{#1}-\eq{#2}}
\def\INCLUDE#1{\typeout{:<+ #1.tex}\include{#1}\typeout{:<-}}
\newcommand{\qed}{\hfill $\Box$}
\newcommand{\qedskip}{\hfill $\Box$\medskip}
\newcommand{\proof}{\noindent {\sc Proof:\ }}
\newcommand{\be}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\dt}{\mathfrak{d}}

\newcommand{\const}{\mbox{\rm const}} %constants

\newcommand{\ptcheck}[1]{{\color{darkgreen}\mnotex{ptc : checked on #1}}}
%
%\newcommand{\redc}{\color{red}}
%\newcommand{\bluec}{\color{blue}}


\newcommand{\blueadd}[2]{\blue{\ptcr{addition or change on #1} #2}}

\newcommand{\redac}[1]{{\blue{\ptc{addition or change on #1} }}
\color{red}}

\newcommand{\topom}[1]{{\red{\ptc{topology addition or change on #1; higher genus needs adding} }}
\color{darkgreen}}
\newcommand{\topo}[1]{{\blue{\ptc{topology addition or change on #1} }}
\color{darkgreen}}

\newcommand{\blueac}[1]{{\blue{\ptc{addition or change on #1} }}\color{blue}}
%\renewcommand{\redad}[2]{#2}

\input{JHmacros}

\newcommand{\ptcnn}[1]{\mnotex{ {  #1}}}
\newcommand{\EdQuery}{\color{blue} \ptcnn{addition addressing queries of the   referees}}

\newcommand{\spaceD}{{ D}}
\newcommand{\zspaceD}{ {\mathring D}}

\newcommand{\mcC}{\mycal C}
\newcommand{\mcE}{\mycal E}
\newcommand{\mcH}{\mycal H}
\newcommand{\deltagone}{\delta \overset{\mbox{\tiny (-1)}}{g}}
\newcommand{\gone}{\overset{\mbox{\tiny (-1)}}{g}}
\newcommand{\gtwo}{\overset{\mbox{\tiny (-2)}}{g}}
\newcommand{\gmone}{\overset{\mbox{\tiny (1)}}{g}}
\newcommand{\gmtwo}{\overset{\mbox{\tiny (2)}}{g}}
\newcommand{\deltagzero}{\overset{\mbox{\tiny (0)}}{\blue{h}}}
\newcommand{\deltagmone}{\overset{\mbox{\tiny (1)}}{\blue{h}}}
\newcommand{\deltagmtwo}{\overset{\mbox{\tiny (2)}}{\blue{h}}}
\newcommand{\gzero}{\overset{\mbox{\tiny (0)}}{g}}

\newcommand{\nobarg}{\blue{g}}



\newcommand{\tL}{\tilde L}
\newcommand{\tH}{\tilde H}

\newcommand{\Lie}{{\mathcal{L}}}

%\newcommand{\redad}[2]{\blue{\jh{change or addition or rewording on #1} #2}}
%\newcommand{\reda}[1]{\jhr{addition or rewording or rearrangement}{ #1}}
%\newcommand{\added}[2]{\jhr{addition or rewording or rearrangement on #1 }{ #2}}
%\newcommand{\reject}{\jhr{remove eject}\eject}
\newcommand{\jh}[1]{\mnotex{{\bf jh:} {  #1}}}
\newcommand{\jhr}[1]{\mnotex{{\bf jh:} {\color{red} #1}}}
\newcommand{\jhbr}[1]{\mnotex{{\bf jh:} {\color{blue} #1}}}
\newcommand{\jhb}[1]{\mnotex{{\bf jh:} {\color{blue} #1}}}
%\newcommand{\change}[1]{{\color{red} #1}\jhr{changed}}
%\newcommand{\add}[1]{{\color{red} #1}\jhr{added}}
%\newcommand{\redadd}[2]{\blue{\jhr{addition or change on #1} #2}}
% ---- TS macros ----
%----- Added 30 XII 20 ----
\newcommand\doubleoverline[1]{\overline{\overline{#1}}}
\newcommand{\zhTBI}{\overline{h}}
\newcommand{\zhTBII}{\doubleoverline{h}}
%----- END Added 30 XII 20 ----
\newcommand{\TSphi}{\blue{\phi}}
\newcommand{\TSpi}{\blue{\pi}}
\newcommand{\TSa}{\blue{a}}
\newcommand{\TSb}{\blue{b}}
\newcommand{\TStphi}{\blue{{\tilde\TSphi}}}
\newcommand{\TStpi}{\blue{{\tilde\TSpi}}}
\newcommand{\tscom}[1]{\mnotex{{\bf ts:} {  #1}}}
\newcommand{\tscomr}[1]{\mnotex{{\bf ts:} {  #1}}}
\newcommand{\tscomc}[1]{\mnotex{{\bf ts check:} {  #1}}}
\newcommand{\TSF}{\blue{\mathcal{F}}}
\newcommand{\TSA}{\blue{A}}
\newcommand{\TSj}{\blue{j}}
\newcommand{\TSn}{\blue{n}}
\newcommand{\SET}{\blue{\mathcal{T}}}
\newcommand{\TSxip}{\blue{\zeta}}
\newcommand{\TSxi}{\blue{\xi}}
\newcommand{\TSr}{\blue{r}}
\newcommand{\TSu}{\blue{u}}
\newcommand{\TSoxi}{\blue{\mathring \TSxi}}
\newcommand{\TSoLie}{\blue{\mathring \Lie}}
%\newcommand{\TSgreen}{\color{green!40!black}}
\newcommand{\TSgreen}{}
%\newcommand{\TSred}{\color{green!70!black}}%{\color{red!80!black}}
\newcommand{\TSred}{}
\newcommand{\TSlambden}{\blue{\Pi}}
%\newcommand{\TSblue}{\color{blue!80!green!80!black}}
\newcommand{\TSblue}{}
%\newcommand{\TSgrn}{\color{green!70!black}}
\newcommand{\TSgrn}{}
\newcommand{\tscnew}[1]{\mnotex{\color{blue!80!green!80!black} { \bf ts26XII:} {  #1}}}
\newcommand{\TSY}{\blue{Y}}
\newcommand{\TSzY}{\blue{\check \TSY}}
\newcommand{\TSoY}{\blue{\mathring \TSY}}
\newcommand{\TswY}{\blue{\widetilde \TSY}}
\newcommand {\TSinvg}{\blue{\widetilde g}}
\newcommand{\xione}{\overset{\mbox{\tiny 1}}{\xi}}
\newcommand{\xitwo}{\overset{\mbox{\tiny 2}}{\xi}}
\newcommand{\TSoone}[1]{\overset{\mbox{\tiny (1)}}{#1}}
\newcommand{\TSotwo}[1]{\overset{\mbox{\tiny (2)}}{#1}}
\newcommand{\reghone}{\delta_{1}g^{\mathrm{reg}}}
\newcommand{\reghtwo}{\delta_{2}g^{\mathrm{reg}}}
\newcommand{\dgbar}[1]{\delta_{#1} \overline{g}}
\newcommand{\tshbar}{\overline{h}}
\newcommand{\TSredd}{\color{red}}
\newcommand{\TSg}{\color{green!70!black}}
% ---- End TS macros ---- 
